Towards autonomous ocean observing systems using Miniature Underwater Gliders with UAV deployment and recovery capabilities

This paper presents preliminary results towards the development of an autonomous ocean observing system using Miniature Underwater Gliders (MUGs) that can operate with the support of Unmanned Aerial Vehicles (UAVs) and Unmanned Surface Vessels (USVs) for deployment, recovery, battery charging, and communication relay. The system reduces human intervention to the minimum, revolutionizing the affordability of a broad range of surveillance and data collection operations. The MUGs are equipped with a small Variable Buoyancy System (VBS) composed of a gas filled piston and a linear actuator powered by brushless DC motor and a rechargable lithium ion battery in an oil filled flexible enclosure. By using a fully pressure tolerant electronic design the aim is to reduce the total complexity, weight, and cost of the overall system. A first prototype of the VBS was built and demonstrated in a small aquarium. The electronic components were tested in a pressure testing facility to a minimum of 20bar. Preliminary results are promising and future work will focus on system and weight optimization, UAV deployment/recovery strategies, as well as sea trials to an operating depth of 200m.

==> sections/1_introduction.tex <==
Here goes the introduction

==> sections/2_section.tex <==
With a density close to that of water the MUG will have neutral buoyancy, neither sinking nor floating. With a variable buoyancy system(VBS) the MUG is able to change its volume and therefore change it's buoyancy. This buoyancy change  enables the glider to either sink or float. 
With a pair of wings this vertical motion enables the MUG to glide forwards. Gliding is an advantageous mode of transportation as it is very energy efficient enabling the MUG to stay operational for longer.

The volume change is controlled by a DC motor connected to a linear actuator positioning a piston. The piston position creates air pressure inside the piston housing, ranging from 1 to 10bar. The piston housing is implemented in an oil filled body with a flexible bladder. Changing the piston position displaces up to 100cc oil, which expands the bladder and changes the volume.

The prototype will initially dive to approximately 200m depth. The pressure at this depth trigger the prototype to start rising up again. This cycle of repeated dives will happen over several iterations. After a set amount of iterations the MUG will rise up and await pickup by an AUV.

The MUG is designed with an pressure compensated oil filled housing. This is due to the strict weight, and cost requirements of the OASYS project. The oil filled design cuts the need for heavy pressure housings.)-Rolf/ole 20.06
